Evaluating Time-Dependent Methods and Seasonal Effects in Code Technical Debt Prediction

Background. Code Technical Debt (Code TD) prediction has gained significant attention in recent software engineering research. However, no standardized approach to Code TD prediction fully captures the factors influencing its evolution. Objective. Our study aims to assess the impact of time-dependent models and seasonal effects on Code TD prediction. It evaluates such models against widely used Machine Learning models, also considering the influence of seasonality on prediction performance. Methods. We trained 11 prediction models with 31 Java open-source projects. To assess their performance, we predicted future observations of the SQALE index. To evaluate the practical usability of our TD forecasting model and its impact on practitioners, we surveyed 23 software engineering professionals. Results. Our study confirms the benefits of time-dependent techniques, with the ARIMAX model outperforming the others. Seasonal effects improved predictive performance, though the impact remained modest. \ReviewerA{ARIMAX/SARIMAX models demonstrated to provide well-balanced long-term forecasts. The survey highlighted strong industry interest in short- to medium-term TD forecasts. Conclusions. Our findings support using techniques that capture time dependence in historical software metric data, particularly for Code TD. Effectively addressing this evidence requires adopting methods that account for temporal patterns.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> Section/tables.tex <==
\begin{table}[]
    \small
    \centering
    \begin{tabular}{l|rrrr}
         \textit{Approach} & MAPE (\%) & MAE & MSE & RMSE\\
         \hline
         \textit{ARIMAX} & 63.05 & 38,223.47 & 29,802,328,854.22 & 50,585.49\\
         \textit{ARIMA + LM} & 10.78 & 9,388.33 & 461,969,247.24 & 11,005.16\\
         \textit{MLR} & 5.34 & 4,506.91 & 286,859,313.43 & 7,753.15\\
         \textit{SVM} & 10.35 & 6,128.88 & 236,607,795.97 & 7,892.37\\
         \textit{XGB} & 1.14 & 1,767.13 & 48,676,305.84 & 2,935.08\\
         \textit{RF} & 2.55 & 3,284.07 & 107,028,276.04 & 4,677.44\\
         \textit{SGD} & 4.69 & 4,536.98 & 166,118,809.64 & 6,042.18\\
         \textit{L1} & 6.54 & 6,292.11 & 268,710,483.95 & 7,697.58\\
         \textit{L2} & 5.24 & 4,684.03 & 170,294,850.98 & 6,218.74\\
         \hline
    \end{tabular}
    \captionsetup{font=small, belowskip=0pt}
    \caption{Performance results from the considered models for the aggregated results of the used 28 considering the biweekly data collection.}
    \label{tab:biweeklyPerformance}
\end{table}



\begin{table}[]
    \small
    \centering
    \begin{tabular}{l|rrrr}
         \textit{Approach} & MAPE (\%) & MAE & MSE & RMSE\\
         \hline
         \textit{ARIMAX} & 21.12 & 18,019.65 & 2,911,197,432.08 & 29,234.19\\
         \textit{ARIMA + LM} & 11.95 & 10,838.01 & 648,407,035.87 & 12,471.43\\
         \textit{MLR} & 5.36 & 5,437.44 & 356,416,553.24 & 7,705.89\\
         \textit{SVM} & 11.42 & 8,811.59 & 541,443,752.24 & 10,667.19\\
         \textit{XGB} & 1.87 & 3,002.36 & 100,337,034.08 & 4,247.42\\
         \textit{RF} & 4.15 & 5,895.89 & 273,522,321.72 & 7,106.93\\
         \textit{SGD} & 4.95 & 5,021.56 & 206,481,655.06 & 6,573.36\\
         \textit{L1} & 7.61 & 7,446.37 & 365,194,175.58 & 8,844.68\\
         \textit{L2} & 6.04 & 5,710.35 & 237,312,213.97 & 7,266.75\\
         \hline
    \end{tabular}
    \captionsetup{font=small}
    \caption{Performance results from the considered predictive models for the aggregated results of the used 28 considering the monthly data collection.}
    \label{tab:monthlyPerformance}
\end{table}

\begin{table}[]
    \small
    \centering
    \begin{tabular}{l|rrrr}
         \textit{Approach} & MAPE (\%) & MAE & MSE & RMSE\\
         \hline
         \textit{MLR} & 6.81 & 4,110.55 & 105,045,073.13 & 5,557.14\\
         \textit{SVM} & 13.21 & 4,276.22 & 57,440,211.46 & 5,356.84\\
         \textit{XGB} & 1.71 & 474.09 & 5,238,430.18 & 1,397.68\\
         \textit{RF} & 2.60 & 964.87 & 8,935,388.66 & 1,900.86\\
         \textit{SGD} & 7.54 & 4,901.81 & 149,332,700.63 & 6,405.58\\
         \textit{L1} & 9.12 & 6,071.25 & 205,929,634.92 & 7,604.60\\
         \textit{L2} & 7.75 & 4,712.63 & 127,660,501.48 & 6,135.45\\
         \hline
    \end{tabular}
    \captionsetup{font=small}
    \caption{Performance results from the ML models for the aggregated results of the used 28 considering the originally collected data.}
    \label{tab:completePerformance}
\end{table}



  \begin{table*}[] 
    \tiny
    \centering
    \begin{tabular}{@{}p{0.8cm}p{0.2cm}p{0.8cm}p{0.8cm}cccccccccccc@{}}
        \hline
        \multirow{2}{*}{\shortstack{\textbf{Apache}\\ \textbf{projects}}} & \multicolumn{5}{c}{\textbf{Complete data}} & \multicolumn{5}{c}{\textbf{Monthly data}} & \multicolumn{5}{c}{\textbf{Biweekly data}}\\
        \cline{2-16} 
         & \textbf{\#} & \textbf{Timeframe} & \textbf{Min/Max \textit{SI}} & \textbf{Mean \textit{SI}} & \textbf{Std \textit{SI}} & \textbf{\#} & \textbf{Timeframe} & \textbf{Min/Max \textit{SI}} & \textbf{Mean \textit{SI}} & \textbf{Std \textit{SI}} & \textbf{\#} & \textbf{Timeframe} & \textbf{Min/Max \textit{SI}} & \textbf{Mean \textit{SI}} & \textbf{Std \textit{SI}}\\
         \hline
        \textit{archiva} & 1,630 & \shortstack{2005/11/28\textminus\\2012/02/24} & 0\textminus172,634 & 71,068.43 & 34,802.64 & 65 & \shortstack{2005/11/28\textminus\\2012/02/08} & 0\textminus116,422 & 68,923.57 & 32,639.24 & 136 & \shortstack{2005/11/28\textminus\\2012/02/16} & 0-121,632 & 68,915.88 & 31,354.32\\
        \textit{batik} & 941 & \shortstack{2000/10/11\textminus\\2002/08/13}& 65,831\textminus175,362& 132,110.99 & 29,957.39 & 21 & \shortstack{2000/10/11\textminus\\2002/07/18} & 71,725\textminus174,077 & 138,099.86 & 30,581.03 & 44 & \shortstack{2000/10/11\textminus\\2002/08/12} & 71,725\textminus174,968 & 140,550.52 & 29,246.41\\
        \textit{bcel} & 291 & \shortstack{2001/10/29\textminus\\2018/04/19} & 47,854\textminus59,608 & 54,304.45 & 3,262.03 & 173 & \shortstack{2001/10/29\textminus\\2018/04/18} & 47,869\textminus58,821 & 54,347.6 & 3,222.63 & 394 & \shortstack{2001/10/29\textminus\\2018/04/18} & 47,869\textminus58,821 & 54,425.75 & 3,233.31\\
        \textit{beanutils} & 324 & \shortstack{2001/03/27\textminus\\2018/10/08} & 1,380\textminus58,250 & 39,024.68 & 14,345.7 & 190 & \shortstack{2001/03/27\textminus\\2018/10/04} & 1,380\textminus58,142 & 47,056.63 & 12,111.02 & 427 & \shortstack{2001/03/27\textminus\\2018/10/04} & 1,380\textminus58,142 & 47,154.16 & 11,838.92\\
        %\textit{cayenne} & 353 & \shortstack{2007/01/21\textminus\\2008-07-05} & 179,813\textminus223,285 & 205,410.63 & 12,555.02 & 17 & %\shortstack{2007/01/21\textminus\\2008/06/25} & 179,813\textminus222,828 & 203,313.71 & 13,480.91 & 33 & \shortstack{2007/01/21\textminus\\2008/07/02} & %179,813\textminus222,875 & 203,402 & 13,343.88\\
        \textit{cocoon} & 2,311 & \shortstack{2003/03/09\textminus\\2007/02/04} & 64,810\textminus286,277 & 183,528.33 & 65,634.23 & 46 & \shortstack{2003/03/09\textminus\\2007/01/17} & 66,640\textminus282,280 & 181,403.89 & 75,407.17 & 95 & \shortstack{2003/03/09\textminus\\2007/02/01} & 65,370\textminus283,313 & 179,950.98 & 73,979.89\\
        \textit{codec} & 229 & \shortstack{2003/05/14\textminus\\2018/05/30} & 2,078\textminus17,707 & 10,618.46 & 4,566.86 & 164 & \shortstack{2003/05/14\textminus\\2018/05/29} & 2,088\textminus17,365 & 10,216.42 & 4,595.29 & 365 & \shortstack{2003/05/14\textminus\\2018/05/29} & 2,078\textminus17,707 & 10,317.17 & 4,553.04\\
        \textit{collections} & 729 & \shortstack{2001/04/14\textminus\\2016/08/04} & 1,494\textminus70,377 & 40,863.99 & 17,315.04 & 155 & \shortstack{2001/04/14\textminus\\2016/08/04} & 1,504\textminus68,115 & 46,947.96 & 13,179.77 & 349 & \shortstack{2001/04/14\textminus\\2016/08/04} & 1,504\textminus67,959 & 47,376.93 & 12,688.5\\
        \textit{commons-cli} & 240 & \shortstack{2002/06/10\textminus\\2017/03/25} & 0\textminus17,714 & 8,610.26 & 4,769.96 & 162 & \shortstack{2002/06/10\textminus\\2017/02/25} & 0\textminus17,519 & 8,280.54 & 3,799.7 & 365 & \shortstack{2002/06/10\textminus\\2017/03/25} & 0\textminus17,519 & 8,281.76 & 3,743.26\\
        \textit{commons-exec} & 100 & \shortstack{2005/08/05\textminus\\2017/10/08} & 2,126\textminus5,537 & 3,637.93 & 915.7 & 136 & \shortstack{2005/08/05\textminus\\2017/10/08} & 2,258\textminus5,537 & 3,908.03 & 1,046.64 & 303 & \shortstack{2005/08/05\textminus\\2017/10/08} & 2,126\textminus5,537 & 3,875.63 & 1,040.7\\
        \textit{commons-fileupload} & 88 & \shortstack{2002/07/17\textminus\\2014/12/02} & 768\textminus6,107 & 3,687.43 & 1,718.72 & 140 & \shortstack{2002/07/17\textminus\\2014/11/11} & 788\textminus5,698 & 4,291.84 & 1,315.21 & 312 & \shortstack{2002/07/17\textminus\\2014/12/02} & 788\textminus5,848 & 4,289.05 & 1,299.02\\
        \textit{commons-io} & 396 & \shortstack{2002/01/26\textminus\\2017/11/16} & 249\textminus42,328 & 15,782.15 & 8,402.13 & 160 & \shortstack{2002/01/26\textminus\\2017/11/16} & 249\textminus42,328 & 18,969.51 & 10,419.96 & 361 & \shortstack{2002/01/26\textminus\\2017/11/16} & 249\textminus42,328 & 19,134.19 & 10,127.72\\
        \textit{commons-jelly} & 311 & \shortstack{2002/02/11\textminus\\2017/09/01} & 1,209\textminus42,910 & 24,178.3 & 11,563.02 & 182 & \shortstack{2002/02/11\textminus\\2017/09/01} & 1,209\textminus42,910 & 40,079.1 & 6,850.43 & 394 & \shortstack{2002/02/11\textminus\\2017/09/01} & 1,209\textminus42,910 & 40,191.97 & 6,437.27\\
        \textit{commons-jexl} & 351 & \shortstack{2002/04/26\textminus\\2018/01/21} & 3,338\textminus20,048 & 12,831.38 & 5,562.45 & 164 & \shortstack{2002/04/26\textminus\\2018/01/08} & 4,363\textminus19,994 & 14,537.46 & 4,414.14 & 368 & \shortstack{2002/04/26\textminus\\2018/01/08} & 3,567\textminus20,040 & 14,604.83 & 4,423.21\\
        \textit{configuration} & 764 & \shortstack{2003/12/24\textminus\\2018/09/16} & 4,498\textminus44,634 & 27,753.8 & 10,462.65 & 147 & \shortstack{2003/12/24\textminus\\2018/09/16} & 5,182\textminus44,634 & 29,485.76 & 9,958.59 & 323 & \shortstack{2003/12/24\textminus\\2018/09/16} & 4,890\textminus44,634 & 29,923.07 & 9,817.25\\
        %\textit{daemon} & 28 & \shortstack{2003/09/27\textminus\\2017/11/02} & 2,290\textminus4,168 & 3,132.96 & 652.03 & 168 & %\shortstack{2003/09/27\textminus\\2017/10/20} & 2,290\textminus4,062 & 3,150.46 & 774.87 & 362 & \shortstack{2003/09/27\textminus\\2017/10/20} & %2,290\textminus4,062 & 3,147.5 & 773.37\\
        \textit{dbcp} & 298 & \shortstack{2001/04/15\textminus\\2016/11/08} & 5,364\textminus19,459 & 13,569.51 & 3,505.79 & 168 & \shortstack{2001/04/15\textminus\\2016/11/02} & 5,364\textminus19,386 & 13,625.74 & 3,445.22 & 368 & \shortstack{2001/04/15\textminus\\2016/11/02} & 5,364\textminus19,319 & 13,635.91 & 3,375.99\\
        \textit{dbutils} & 63 & \shortstack{2003/11/09\textminus\\2015/04/20} & 3,357\textminus7,954 & 4,935.3 & 1,339.41 & 129 & \shortstack{2003/11/09\textminus\\2015/04/13} & 3,357\textminus6,782 & 4,670.78 & 1,192.73 & 288 & \shortstack{2003/11/09\textminus\\2015/04/13} & 3,357\textminus6,782 & 4,696.2 & 1,192.2\\
        \textit{digester} & 340 & \shortstack{2001/05/12\textminus\\2017/08/25} & 20\textminus31,542 & 13,420.25 & 6,824.58 & 179 & \shortstack{2001/05/12\textminus\\2017/08/25} & 20\textminus31,525 & 21,636.41 & 9,355.68 & 397 & \shortstack{2001/05/12\textminus\\2017/08/25} & 20\textminus31,525 & 21,627.09 & 6,699.97\\
        \textit{felix} & 1,149 & \shortstack{2005/08/16\textminus\\2009/07/15} & 22,667\textminus283,638 & 144,965.65 & 73,748.93 & 44 & \shortstack{2005/08/16\textminus\\2009/07/15} & 22,667\textminus283,530 & 121,831.43 & 75,758.16 & 88 & \shortstack{2005/08/16\textminus\\2009/07/10} & 24,405\textminus265,380 & 120,187.45 & 74,219.65\\
        \textit{hive} & 3,001 & \shortstack{2008/09/02\textminus\\2015/03/03} & 73,317\textminus701,914 & 434,702.59 & 201,776.41 & 75 & \shortstack{2008/09/02\textminus\\2015/02/23} & 73,332\textminus701,210 & 288,530.53 & 187,519.16 & 154 & \shortstack{2008/09/02\textminus\\2015/02/23} & 73,332\textminus687,974 & 289,030.01 & 186,604.21\\
        \textit{httpclient} & 902 & \shortstack{2005/12/21\textminus\\2017/05/06} & 55\textminus85,666 & 48,009.34 & 25,366.31 & 114 & \shortstack{2005/12/21\textminus\\2017/05/01} & 55\textminus85,666 & 49,809.22 & 26,021.89 & 244 & \shortstack{2005/12/21\textminus\\2017/05/01} & 55\textminus85,666 & 49,204.92 & 25,700.54\\
        \textit{httpcore} & 666 & \shortstack{2005/02/19\textminus\\2017/05/04} & 547\textminus86,264 & 36,144.59 & 24,796.72 & 131 & \shortstack{2005/02/19\textminus\\2017/05/01} & 547\textminus81,133 & 47,584.99 & 19,595.95 & 284 & \shortstack{2005/02/19\textminus\\2017/05/04} & \textminus83,497 & 47,663.48 & 19,368.05\\
        \textit{jxpath} & 148 & \shortstack{2001/09/03\textminus\\2018/05/15} & 23,071\textminus32,029 & 28,448.3 & 2,499.92 & 188 & \shortstack{2001/09/03\textminus\\2018/05/15} & 24,708\textminus32,029 & 29,012.59 & 1,840.07 & 422 & \shortstack{2001/09/03\textminus\\2018/05/15} & 23,071\textminus32,029 & 29,032.03 & 1,896.42\\
        \textit{net} & 543 & \shortstack{2002/04/03\textminus\\2018/10/05} & 12,516\textminus34,898 & 23,536.09 & 3,347.05 & 169 & \shortstack{2002/04/03\textminus\\2018/10/05} & 12,706\textminus30,433 & 24,282.76 & 4,163.03 & 374 & \shortstack{2002/04/03\textminus\\2018/10/05} & 12,706\textminus30,433 & 24,372.49 & 4,088.35\\
        %\textit{ognl} & 72 & \shortstack{2011/05/11\textminus\\2018/06/08} & 20,410\textminus34,077 & 27,277.78 & 5,615.44 & 85 & %\shortstack{2011/05/11\textminus\\2018/06/08} & 20,437\textminus34,006 & 26,773.85 & 1,855.06 & 183 & \shortstack{2011/05/11\textminus\\2018/06/08} & %20,444\textminus34,006 & 26,711.87 & 1,716.58\\
        \textit{santuario} & 914 & \shortstack{2001/1001\textminus\\2018/10/15} & 2,201\textminus126,431 & 71,471.9 & 25,715.67 & 162 & \shortstack{2001/10/01\textminus\\2018/10/01} & 2,201\textminus126,431 & 80,389.48 & 27,220.1 & 371 & \shortstack{2001/10/01\textminus\\2018/10/15} & 2,201\textminus126,431 & 82,370.35 & 27,045.79\\
        \textit{thrift} & 145 & \shortstack{2008/05/16\textminus\\2012/10/26} & 0\textminus21,395 & 15,965.12 & 3,629.11 & 42 & \shortstack{2008/05/16\textminus\\2012/10/09} & 0\textminus21,026 & 16,485.57 & 4,347.45 & 96 & \shortstack{2008/05/16\textminus\\2012/10/26} & 0\textminus21,395 & 16,756.9 & 4,056.79\\
        \textit{validator} & 249 & \shortstack{2002/01/06\textminus\\2018/10/07} & 39\textminus17,541 & 17,850.83 & 4,089.55 & 184 & \shortstack{2002/01/06\textminus\\2018/09/29} & 39\textminus17,541 & 12,725.59 & 3,615.91 & 407 & \shortstack{2002/01/06\textminus\\2018/09/29} & 39\textminus17,541 & 12,791.12 & 3,548.96\\
        \textit{vfs} & 428 & \shortstack{2002/07/17\textminus\\2018/07/23} & 4,175\textminus29,340 & 17,850.83 & 7,192.67 & 168 & \shortstack{2002/07/17\textminus\\2018/07/23} & 4,175\textminus29,340 & 21,430.57 & 6,168 & 373 & \shortstack{2002/07/17\textminus\\2018/07/23} & 4,175\textminus29,340 & 21,667.49 & 5,862.13\\
        \textit{zookeeper} & 58 & \shortstack{2014/07/23\textminus\\2016/12/21} & 57,033\textminus64,173 & 60,067.5 & 1,925.89 & 24 & \shortstack{2014/07/23\textminus\\2016/11/24} & 57,033\textminus64,090 & 60,116.29 & 1,971.02 & 52 & \shortstack{2014/07/23\textminus\\2016/12/20} & 57,033\textminus64,173 & 60,149.95 & 1,996.84\\
        \hline
 
    \end{tabular}
    \captionsetup{font=small}
    \caption{Descriptive statistics from the projects used in the analysis.}
    \label{tab:descriptiveStats}
\end{table*}



\begin{table*}[h!] 
    \centering
    \small
    \begin{tabular}{@{}l|rrr|rrrrr@{}}
        \hline
        Variable & Mean value & St.deviation & Min value & Lower quartile & Median value & Upper quartile & Max value & Skewness\\
        \hline
        SQALE index & 137,726.34 & 169,926.75 & 0 & 24,377.5 & 72,981 & 182,132.25 & 701,914 & 1.87\\
        S1213 & 739.99 & 1,349.67 & 0 & 38 & 152 & 579 & 6,106 & 2.22\\
        RedundantThrows DeclarationCheck & 344.95 & 509.21 & 0 & 15 & 113 & 340 & 2,200 & 1.91\\
        S00117 & 1,082.47 & 2,379.79 & 0 & 7 & 55 & 383 & 10,395 & 2.3\\
        S00122 & 401.83 & 657.81 & 0 & 1 & 67 & 585 & 4,119 & 2.55\\
        S1488 & 87.76 & 163.26 & 0 & 4 & 20 & 81 & 1,196 & 2.85\\
        S1905 & 73.69 & 148.02 & 0 & 1 & 12 & 44 & 575 & 2.26\\
        UselessImportCheck & 629.85 & 1,401.83 & 0 & 7 & 42 & 151 & 7,928 & 2.58\\
        DuplicatedBlocks & 333.23 & 510.3 & 0 & 40 & 142 & 305 & 3,099 & 2.52\\
        S1226 & 212.21 & 293.13 & 0 & 18 & 62 & 330 & 1,479 & 1.91\\
        S00112 & 472.76 & 847.98 & 0 & 58 & 183 & 374 & 4,987 & 3.01\\
        S1155 & 86.23 & 168.93 & 0 & 2 & 12 & 67 & 933 & 2.49\\
        S00108 & 97.23 & 127.71 & 0 & 4 & 62 & 127 & 739 & 1.95\\
        S1151 & 471.73 & 1,006.97 & 0 & 2 & 26 & 200 & 3,699 & 2.25\\
        S1132 & 289.38 & 481.4 & 0 & 20 & 57 & 436 & 3,587 & 2.94\\
        S1481 & 132.35 & 274.22 & 0 & 5 & 18 & 71 & 1,600 & 2.75\\
        \hline
    \end{tabular}
    \captionsetup{font=footnotesize}
    \caption{Descriptive statistics from the resulting model variables.}
    \label{tab:modelVariables}
\end{table*}


\onecolumn
\scriptsize
\begin{longtable}{llllllllllll} % Define table columns


\hline
\textbf{Project} & \textbf{Model} & \textbf{\begin{tabular}[c]{@{}l@{}}Seriali\\ zation\end{tabular}} & \textbf{p} & \textbf{d} & \textbf{q} & \textbf{P} & \textbf{D} & \textbf{Q} & \textbf{m} & \textbf{AIC} & \textbf{Regressors} \\ 
\hline
\endfirsthead

% Define the header for subsequent pages
\hline
\textbf{Project} & \textbf{Model} & \textbf{\begin{tabular}[c]{@{}l@{}}Seriali\\ zation\end{tabular}} & \textbf{p} & \textbf{d} & \textbf{q} & \textbf{P} & \textbf{D} & \textbf{Q} & \textbf{m} & \textbf{AIC} & \textbf{Regressors} \\ 
\hline
\endhead

% Define footer (optional, can remove if not needed)
\hline
\multicolumn{12}{r}{\textit{Continued on next page}} \\ 
\hline
\endfoot

\hline
\endlastfoot

archiva          & Arimax         & monthly                                                           & 0          & 0          & 1          &            &            &            & 12         & 777.97       & \begin{tabular}[c]{@{}l@{}}S1213, S1192, RedundantThrowsDeclarationCheck, S00117, \\ S1488, DuplicatedBlocks, S1186, S1132\end{tabular}                                                                                                                     \\
bcel             & Arimax         & monthly                                                           & 1          & 0          & 1          &            &            &            & 12         & 1194.46      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S00122, S1488, \\ DuplicatedBlocks, S134, S1066, MethodCyclomaticComplexity, \\ S00112, S00108, S1186, S1151, S1132\end{tabular}                                                      \\
codec            & Arimax         & monthly                                                           & 0          & 1          & 1          &            &            &            & 12         & 1312.76      & \begin{tabular}[c]{@{}l@{}}ModifiersOrderCheck, S1192, RedundantThrowsDeclarationCheck, \\ S00117, DuplicatedBlocks, S134, MethodCyclomaticComplexity, \\ S1226, S00112, S00108, S1186, S1151, S1132\end{tabular}                                           \\
collections      & Arimax         & monthly                                                           & 0          & 0          & 1          &            &            &            & 12         & 1634.78      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S00117, S00122, S1488, \\ DuplicatedBlocks, S134, MethodCyclomaticComplexity, \\ S1226, S00112, S1155, S00108, S1186, S1151, S1132\end{tabular}                                                      \\
cli*             & Arimax         & monthly                                                           & 0          & 0          & 1          &            &            &            & 12         & 1775.66      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S134, S1066, \\ S1226, S00112, S1186, S1132\end{tabular}                                                                                                                              \\
exec*            & Arimax         & monthly                                                           & 1          & 1          & 0          &            &            &            & 12         & 903.43       & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S1488, \\ DuplicatedBlocks, S134, MethodCyclomaticComplexity, \\ S1226, S00112, S1155, S00108, S1186, S1151, S1132\end{tabular}                                                       \\
configuration    & Arimax         & monthly                                                           & 0          & 1          & 1          &            &            &            & 12         & 1533.28      & \begin{tabular}[c]{@{}l@{}}ModifiersOrderCheck, RedundantThrowsDeclarationCheck, \\ S00122, MethodCyclomaticComplexity, S00112, S00108\end{tabular}                                                                                                         \\
dbcp             & Arimax         & monthly                                                           & 1          & 0          & 1          &            &            &            & 12         & 1352.23      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, DuplicatedBlocks, \\ S1066, S00112, S1155, S00108\end{tabular}                                                                                            \\
hive             & Arimax         & monthly                                                           & 0          & 0          & 2          &            &            &            & 12         & 885.95       & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, S1488, S1226, S1186, \\ S1151, S1132\end{tabular}                                                                                                         \\
httpclient       & Arimax         & monthly                                                           & 0          & 0          & 1          &            &            &            & 12         & 1301.53      & \begin{tabular}[c]{@{}l@{}}ModifiersOrderCheck, S1192, RedundantThrowsDeclarationCheck, \\ S134, S1186\end{tabular}                                                                                                                                         \\
httpcore         & Arimax         & monthly                                                           & 2          & 2          & 1          &            &            &            & 12         & 1374.66      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S00122, \\ S1488, DuplicatedBlocks, S134, S1066, \\ MethodCyclomaticComplexity, S1226, S00112, S1155, S00108\end{tabular}                                                             \\
jxpath           & Arimax         & monthly                                                           & 0          & 0          & 1          &            &            &            & 12         & 1592.83      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S00117, S00122, S1488, \\ DuplicatedBlocks, S134, S1066, MethodCyclomaticComplexity, \\ S1226, S00112, S1155, S1186, S1151, S1132\end{tabular}                                                       \\
santuario        & Arimax         & monthly                                                           & 0          & 0          & 1          &            &            &            & 12         & 1848.2       & \begin{tabular}[c]{@{}l@{}}S1213, S1192, RedundantThrowsDeclarationCheck, \\ DuplicatedBlocks, S134, S1066, S00112, S00108, S1132\end{tabular}                                                                                                              \\
validator        & Arimax         & monthly                                                           & 1          & 0          & 1          &            &            &            & 12         & 1473.72      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S00122, \\ S1488, DuplicatedBlocks, S134, S1066, S1226, S00112, \\ S1155, S00108, S1186, S1151, S1132\end{tabular}                                                                    \\
archiva          & Arimax         & biweekly                                                          & 1          & 0          & 1          &            &            &            & 26         & 1599.0       & S1192, S1488, S1226, S1155, S1186                                                                                                                                                                                                                           \\
bcel             & Arimax         & biweekly                                                          & 1          & 1          & 1          &            &            &            & 26         & 2459.66      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, S00117, S00122, \\ S1488, DuplicatedBlocks, S134, S1066, \\ MethodCyclomaticComplexity, S1226, S00112, S1155, \\ S00108, S1186, S1151, S1132\end{tabular} \\
codec            & Arimax         & biweekly                                                          & 1          & 0          & 1          &            &            &            & 26         & 2815.72      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, \\ RedundantThrowsDeclarationCheck, S00122, \\ DuplicatedBlocks, S134, MethodCyclomaticComplexity, \\ S1226, S1186\end{tabular}                                                                      \\
collections      & Arimax         & biweekly                                                          & 5          & 5          & 1          &            &            &            & 26         & 3663.77      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, DuplicatedBlocks, \\ S1066, MethodCyclomaticComplexity, S1155, S1151\end{tabular}                                                                         \\
cli*             & Arimax         & biweekly                                                          & 1          & 0          & 0          &            &            &            & 26         & 4032.23      & \begin{tabular}[c]{@{}l@{}}ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, S00117, \\ DuplicatedBlocks, S134, S1066, S1226, S00112, \\ S1155, S1151, S1132\end{tabular}                                                                     \\
exec*            & Arimax         & biweekly                                                          & 2          & 0          & 0          &            &            &            & 26         & 1799.48      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, S00117, S1488, \\ DuplicatedBlocks, S134, S1066, \\ MethodCyclomaticComplexity, S1226, S1155, S00108, \\ S1186, S1151, S1132\end{tabular}                 \\
configuration    & Arimax         & biweekly                                                          & 2          & 0          & 0          &            &            &            & 26         & 3113.02      & \begin{tabular}[c]{@{}l@{}}S1213, RedundantThrowsDeclarationCheck, S00117, S00122, \\ S1488, S134, MethodCyclomaticComplexity, S1226, S00112, \\ S00108, S1186, S1132\end{tabular}                                                                          \\
dbcp             & Arimax         & biweekly                                                          & 2          & 1          & 0          &            &            &            & 26         & 1728.23      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00122, S1488, \\ DuplicatedBlocks, S134, S1066, \\ MethodCyclomaticComplexity, S00112, S1155, S1186, \\ S1151, S1132\end{tabular}                                                            \\
hive             & Arimax         & biweekly                                                          & 0          & 0          & 1          &            &            &            & 26         & 1796.37      & \begin{tabular}[c]{@{}l@{}}S1213, S1192, RedundantThrowsDeclarationCheck, S00122, \\ DuplicatedBlocks, S134, S00112, S1155, S00108, S1151, S1132\end{tabular}                                                                                               \\
httpclient       & Arimax         & biweekly                                                          & 0          & 0          & 1          &            &            &            & 26         & 2692.53      & \begin{tabular}[c]{@{}l@{}}S1192, S00117, S1066, MethodCyclomaticComplexity, \\ S00112, S1155, S1132\end{tabular}                                                                                                                                           \\
httpcore         & Arimax         & biweekly                                                          & 1          & 1          & 1          &            &            &            & 26         & 2931.74      & \begin{tabular}[c]{@{}l@{}}S1192, RedundantThrowsDeclarationCheck, S1488, S134, \\ S1066, MethodCyclomaticComplexity, S1186, S1151, S1132\end{tabular}                                                                                                      \\
jxpath           & Arimax         & biweekly                                                          & 0          & 3          & 1          &            &            &            & 26         & 3064.28      & \begin{tabular}[c]{@{}l@{}}S1213, S1192, S00117, S00122, S1488, DuplicatedBlocks, \\ S134, MethodCyclomaticComplexity, S1226, S00112, S1155, \\ S00108, S1132\end{tabular}                                                                                  \\
santuario        & Arimax         & biweekly                                                          & 0          & 2          & 1          &            &            &            & 26         & 4123.08      & \begin{tabular}[c]{@{}l@{}}S1213, RedundantThrowsDeclarationCheck, S00117, S134, \\ S00112, S1186, S1151\end{tabular}                                                                                                                                       \\
validator        & Arimax         & biweekly                                                          & 1          & 0          & 1          &            &            &            & 26         & 2981.88      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S00122, \\ S1488, DuplicatedBlocks, S134, S1226, S00112, S1155, S1186\end{tabular}                                                                                                    \\
archiva          & Sarimax        & monthly                                                           & 0          & 1          & 2          & 0          & 0          & 0          & 12         & 761.79       & \begin{tabular}[c]{@{}l@{}}S1192, S00122, S1488, MethodCyclomaticComplexity, \\ S00112, S00108, S1186, S1151\end{tabular}                                                                                                                                   \\
bcel             & Sarimax        & monthly                                                           & 1          & 0          & 1          & 0          & 0          & 0          & 12         & 1194.46      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S00122, S1488, \\ DuplicatedBlocks, S134, S1066, MethodCyclomaticComplexity, \\ S00112, S00108, S1186, S1151, S1132\end{tabular}                                                      \\
codec            & Sarimax        & monthly                                                           & 1          & 0          & 1          & 0          & 1          & 0          & 12         & 1309.26      & \begin{tabular}[c]{@{}l@{}}ModifiersOrderCheck, S1192, RedundantThrowsDeclarationCheck, \\ S00117, DuplicatedBlocks, S134, MethodCyclomaticComplexity, \\ S1226, S00112, S00108, S1186, S1151, S1132\end{tabular}                                           \\
collections      & Sarimax        & monthly                                                           & 2          & 2          & 1          & 0          & 0          & 0          & 12         & 1635.7       & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, S00117, S00122, \\ DuplicatedBlocks, S134, MethodCyclomaticComplexity, \\ S1226, S00112, S1155, S00108, S1186, S1151\end{tabular}                         \\
cli*             & Sarimax        & monthly                                                           & 0          & 0          & 1          & 0          & 0          & 0          & 12         & 1775.66      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S134, S1066, \\ S1226, S00112, S1186, S1132\end{tabular}                                                                                                                              \\
exec*            & Sarimax        & monthly                                                           & 0          & 4          & 1          & 0          & 0          & 0          & 12         & 935.31       & S1213, MethodCyclomaticComplexity, S00108, S1151, S1132                                                                                                                                                                                                     \\
configuration    & Sarimax        & monthly                                                           & 0          & 1          & 1          & 0          & 0          & 0          & 12         & 1536.79      & \begin{tabular}[c]{@{}l@{}}S1192, RedundantThrowsDeclarationCheck, \\ MethodCyclomaticComplexity, S00108, S1151\end{tabular}                                                                                                                                \\
dbcp             & Sarimax        & monthly                                                           & 1          & 0          & 1          & 0          & 0          & 0          & 12         & 1323.82      & \begin{tabular}[c]{@{}l@{}}S1213, S1192, S00122, DuplicatedBlocks, S134, \\ MethodCyclomaticComplexity, S1226, S00112, S1155\end{tabular}                                                                                                                   \\
hive             & Sarimax        & monthly                                                           & 0          & 0          & 2          & 0          & 0          & 0          & 12         & 885.95       & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, S1488, S1226, S1186, \\ S1151, S1132\end{tabular}                                                                                                         \\
httpclient       & Sarimax        & monthly                                                           & 0          & 0          & 1          & 0          & 0          & 0          & 12         & 1301.53      & \begin{tabular}[c]{@{}l@{}}ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, S134, S1186\end{tabular}                                                                                                                                         \\
httpcore         & Sarimax        & monthly                                                           & 2          & 2          & 1          & 1          & 1          & 0          & 12         & 1376.82      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, S00117, S00122, S1488, \\ DuplicatedBlocks, S134, S1066, MethodCyclomaticComplexity, \\ S1226, S00112, S1155, S00108, S1186, S1151, S1132\end{tabular}    \\
jxpath           & Sarimax        & monthly                                                           & 0          & 0          & 1          & 0          & 0          & 0          & 12         & 1592.83      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S00117, S00122, S1488, \\ DuplicatedBlocks, S134, S1066, MethodCyclomaticComplexity, \\ S1226, S00112, S1155, S1186, S1151, S1132\end{tabular}                                                       \\
santuario        & Sarimax        & monthly                                                           & 0          & 0          & 1          & 0          & 0          & 0          & 12         & 1848.2       & \begin{tabular}[c]{@{}l@{}}S1213, S1192, RedundantThrowsDeclarationCheck, \\ DuplicatedBlocks, S134, S1066, S00112, S00108, S1132\end{tabular}                                                                                                              \\
validator        & Sarimax        & monthly                                                           & 1          & 0          & 1          & 0          & 0          & 0          & 12         & 1460.96      & \begin{tabular}[c]{@{}l@{}}S1213, S00117, S00122, DuplicatedBlocks, S134, S1226, \\ S00112, S1155, S00108, S1132\end{tabular}                                                                                                                               \\
archiva          & Sarimax        & biweekly                                                          & 1          & 0          & 1          & 0          & 0          & 0          & 26         & 1599.0       & S1192, S1488, S1226, S1155, S1186                                                                                                                                                                                                                           \\
bcel             & Sarimax        & biweekly                                                          & 3          & 0          & 1          & 0          & 0          & 0          & 26         & 2460.57      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, S00117, S00122, S1488, \\ DuplicatedBlocks, S134, S1066, MethodCyclomaticComplexity, \\ S1226, S00112, S1155, S00108, S1186, S1151, S1132\end{tabular}    \\
codec            & Sarimax        & biweekly                                                          & 1          & 0          & 0          & 1          & 0          & 0          & 26         & 728.68       & \begin{tabular}[c]{@{}l@{}}S1213, RedundantThrowsDeclarationCheck, S00122, \\ DuplicatedBlocks, S134, MethodCyclomaticComplexity, S1226, S00108\end{tabular}                                                                                                \\
collections      & Sarimax        & biweekly                                                          & 4          & 3          & 1          & 0          & 0          & 0          & 26         & 3693.5       & \begin{tabular}[c]{@{}l@{}}S1213, S1192, DuplicatedBlocks, S134, \\ MethodCyclomaticComplexity, S00112, S00108, S1186\end{tabular}                                                                                                                          \\
cli*             & Sarimax        & biweekly                                                          & 1          & 1          & 1          & 1          & 0          & 0          & 26         & 4031.03      & S00112, S1132                                                                                                                                                                                                                                               \\
exec*            & Sarimax        & biweekly                                                          & 1          & 0          & 1          & 1          & 0          & 0          & 26         & 1900.19      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S1488, \\ DuplicatedBlocks, S134, S1066, MethodCyclomaticComplexity, \\ S1226, S1155, S00108, S1151, S1132\end{tabular}                                                               \\
configuration    & Sarimax        & biweekly                                                          & 3          & 1          & 1          & 0          & 0          & 0          & 26         & 3105.48      & \begin{tabular}[c]{@{}l@{}}S1213, RedundantThrowsDeclarationCheck, S00117, \\ MethodCyclomaticComplexity, S1226, S00108, S1186\end{tabular}                                                                                                                 \\
dbcp             & Sarimax        & biweekly                                                          & 2          & 0          & 1          & 0          & 0          & 0          & 26         & 2703.93      & S1213, DuplicatedBlocks, S134, S1155, S00108, S1186                                                                                                                                                                                                         \\
hive             & Sarimax        & biweekly                                                          & 0          & 0          & 1          & 0          & 0          & 0          & 26         & 1796.37      & \begin{tabular}[c]{@{}l@{}}S1213, S1192, RedundantThrowsDeclarationCheck, S00122, \\ DuplicatedBlocks, S134, S00112, S1155, S00108, S1151, S1132\end{tabular}                                                                                               \\
httpclient       & Sarimax        & biweekly                                                          & 0          & 0          & 1          & 0          & 0          & 0          & 26         & 2693.89      & \begin{tabular}[c]{@{}l@{}}RedundantThrowsDeclarationCheck, S00117, \\ MethodCyclomaticComplexity, S00112, S1155, S1151\end{tabular}                                                                                                                        \\
httpcore         & Sarimax        & biweekly                                                          & 1          & 2          & 1          & 0          & 0          & 0          & 26         & 2921.25      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, \\ RedundantThrowsDeclarationCheck, S1488, DuplicatedBlocks, \\ S134, S1066, S00112, S1155, S00108, S1151\end{tabular}                                                                        \\
jxpath           & Sarimax        & biweekly                                                          & 5          & 0          & 1          & 1          & 0          & 0          & 26         & 3029.53      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S134, S1226, \\ S00112, S1155, S00108, S1186, S1151, S1132\end{tabular}                                                                                                               \\
santuario        & Sarimax        & biweekly                                                          & 2          & 0          & 1          & 0          & 0          & 0          & 26         & 4099.67      & \begin{tabular}[c]{@{}l@{}}S1213, RedundantThrowsDeclarationCheck, S00122, S134, \\ S00112, S1155, S00108, S1186, S1132\end{tabular}                                                                                                                        \\
validator        & Sarimax        & biweekly                                                          & 1          & 0          & 1          & 0          & 0          & 0          & 26         & 3018.51      & \begin{tabular}[c]{@{}l@{}}S1213, ModifiersOrderCheck, S1192, S00117, S00122, \\ DuplicatedBlocks, S134, S1066, S1226, S00112, S00108, S1151\end{tabular}

\\

\end{longtable}

\twocolumn

==> Table/RW_OLD.tex <==
\begin{table*}[]
\tiny
\centering
\label{tab:relatedworks}
\caption{Related work on the existing research on TD prediction \textcolor{red}{TODO: ADD ROW WITH HOW ML HAS USED OR TREATED THE TIME SERIES DATA}}
\begin{tabular}{l|l|c|c|c|c|c|c}
\hline
& \textbf{Tsoukalas et al. \cite{Tsoukalas2020}}   & \textbf{Tsoukalas et al. \cite{tsoukalas2021machine}} & \textbf{Mathioudaki et al. \cite{Mathioudaki2021}}                                     & \textbf{Aversano et al. \cite{Aversano2022}}  & \textbf{Mathioudaki et al. \cite{Mathioudaki2022}} & \textbf{Zozas et al. \cite{Zozas2023}}  & \textbf{Our work}  \\ \hline


\textbf{Seasonality} &   &   &     &   &    &  & ✓  \\ \hline 
\textbf{Feature selection}                                                & Correlation analysis & Hypothesis testing                              &                                                                          & Correlation analysis &                                                                          &                                                                                        & Correlation analysis  \\ 

& backward elimination &&&&& feature importance \\
&&&&&& variance thresolding\\
&&&&&& zero percentage\\

\textbf{\begin{tabular}[c]{@{}l@{}}Hyperparameter \\ tuning\end{tabular}} & \begin{tabular}[c]{@{}c@{}}✓\\ (GridSearchCV)\end{tabular}                                 & \begin{tabular}[c]{@{}c@{}}✓\\ (Grid-search \\ method)\end{tabular}                                & \begin{tabular}[c]{@{}c@{}}✓\\ (Grid-search \\ method)\end{tabular}      &                                                                    & \begin{tabular}[c]{@{}c@{}}✓\\ (ACF, PACF)\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}✓\\ (Backward Stepwise \\ Regression \\ (BSR))\end{tabular} & \begin{tabular}[c]{@{}c@{}}✓\\ (Auto-ARIMA)\end{tabular}                                                                               \\
\textbf{\begin{tabular}[c]{@{}l@{}}Univariate \\ models\end{tabular}}     &                                                                                            & \begin{tabular}[c]{@{}c@{}}✓\\ (Univariate logistic \\ regression)\end{tabular}                    & \begin{tabular}[c]{@{}c@{}}✓\\ (Multi-layer \\ perceptron)\end{tabular}  &                                                                    & \begin{tabular}[c]{@{}c@{}}✓\\ (ARIMA)\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}✓\\ (ARIMA)\end{tabular}                                    & \begin{tabular}[c]{@{}c@{}}✓\\ (ARIMA, SARIMA)\end{tabular}                                                                            \\
\textbf{\begin{tabular}[c]{@{}l@{}}Multivariate \\ models\end{tabular}}   & \begin{tabular}[c]{@{}c@{}}✓\\ (MLR, SGD, SVR...)\end{tabular}                             & \begin{tabular}[c]{@{}c@{}}✓\\ (LR, NB, \\ DT, KNN, \\ SVM, RF, \\ XGB)\end{tabular}               &                                                                          & \begin{tabular}[c]{@{}c@{}}✓\\ (MLR, BDT, \\ RF)\end{tabular}      & \begin{tabular}[c]{@{}c@{}}✓\\ (ARIMAX)\end{tabular}                     &                                                                                        & \begin{tabular}[c]{@{}c@{}}✓\\ (ARIMAX, SARIMAX, \\ MLR,  SGD, \\ SVR, RF, XGB, ...)\end{tabular}                                      \\
\textbf{Industrial survey}                                                & ✓                                                                                          &                                                                                                    &                                                                          &                                                                    &                                                                          & ✓                                                                                      & ✓                                                                                                                                      \\
\textbf{\begin{tabular}[c]{@{}l@{}}Long-term \\ forecasting\end{tabular}} & \begin{tabular}[c]{@{}c@{}}✓\\ (1 to 40 weeks ahead)\end{tabular}                          &                                                                                                    & \begin{tabular}[c]{@{}c@{}}✓\\ (5 to 150 commits \\ ahead)\end{tabular}  &                                                                    & \begin{tabular}[c]{@{}c@{}}✓\\ (4, 8, 12 steps \\ ahead)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}✓\\ (12 iterations \\ ahead)\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}✓\\ (1 to 36 months \\ ahead)\end{tabular}                                                                  \\
\textbf{\begin{tabular}[c]{@{}l@{}}Time Series  \\ models\end{tabular}}   &                                                                                            &                                                                                                    & \begin{tabular}[c]{@{}c@{}}✓\\ (ARIMA)\end{tabular}                      &                                                                    & \begin{tabular}[c]{@{}c@{}}✓\\ (ARIMA, \\ ARIMAX)\end{tabular}           & \begin{tabular}[c]{@{}c@{}}✓\\ (ARIMA)\end{tabular}                                    & \begin{tabular}[c]{@{}c@{}}✓\\ (ARIMAX, ARIMA+LM, \\ SARIMAX, SARIMA+LM)\end{tabular}                                                  \\
\textbf{ML models}                                                        & \begin{tabular}[c]{@{}c@{}}✓\\ (MLR, SGD, SVR...)\end{tabular}                             & \begin{tabular}[c]{@{}c@{}}✓\\ (LR, NB, \\ DT, KNN,\\  SVM, \\ RF, XGB)\end{tabular}               & \begin{tabular}[c]{@{}c@{}}✓\\ (RF)\end{tabular}                         & \begin{tabular}[c]{@{}c@{}}✓\\ (MLR, BDT, \\ RF)\end{tabular}      &                                                                          &                                                                                        & \begin{tabular}[c]{@{}c@{}}✓\\ (MLR, SGD, \\ SVR, RF, XGB, ...)\end{tabular}                                                           \\
\textbf{DL models}                                                        &                                                                                            &                                                                                                    & \begin{tabular}[c]{@{}c@{}}✓\\ (Multi-layer \\ perceptron)\end{tabular}  &                                                                    &                                                                          &                                                                                        &                                                                                                                                        \\
\textbf{Cross-validation}                                                 & \begin{tabular}[c]{@{}c@{}}✓\\ (Walk-Forward \\ Train-Test)\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}✓\\ (Repeated stratified \\ CV)\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}✓\\ (Walk-Forward \\ Train-Test)\end{tabular} & \begin{tabular}[c]{@{}c@{}}✓\\ (Repeated  CV)\end{tabular}         & \begin{tabular}[c]{@{}c@{}}✓\\ (Walk-Forward \\ Train-Test)\end{tabular} & \begin{tabular}[c]{@{}c@{}}✓\\ (Walk-Forward \\ Train-Test)\end{tabular}               & \begin{tabular}[c]{@{}c@{}}✓\\ (Walk-Forward \\ Train-Test)\end{tabular}                                                               \\
\textbf{\begin{tabular}[c]{@{}l@{}}Performance \\ metrics\end{tabular}}   & \begin{tabular}[c]{@{}c@{}}✓\\ (MAPE)\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}✓\\ (Precision, Recall, \\ F2,  AUC, \\ Module inspection)\end{tabular} & \begin{tabular}[c]{@{}c@{}}✓\\ (MAPE, MAE, \\ RMSE)\end{tabular}         & \begin{tabular}[c]{@{}c@{}}✓\\ (RMSE)\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}✓\\ (MAPE, MAE, \\ RMSE)\end{tabular}         & \begin{tabular}[c]{@{}c@{}}✓\\ (MAPE, MAE, \\ RMSE)\end{tabular}                       & \begin{tabular}[c]{@{}c@{}}✓\\ (MAPE, MAE, \\ RMSE)\end{tabular}                                                                       \\
\textbf{Sample size}                                                      & 15 projects                                                                                & 25 projects                                                                                        & 5 projects                                                               & 8 projects                                                         & 5 projects                                                               & 105 projects                                                                           & 14 projects                                                                                                                            \\
\textbf{Results}                                                          & ✓                                                                                          & ✓                                                                                                  & ✓                                                                        & ✓                                                                  & ✓                                                                        & ✓                                                                                      & ✓                                                                                                                                      \\
\textbf{Scripts}                                                          & ✓                                                                                          & ✓                                                                                                  &                                                                          &                                                                    &                                                                          &                                                                                        & ✓                                                                                                                                      \\
\textbf{Datasets}                                                         & ✓                                                                                          & ✓                                                                                                  &                                                                          & ✓                                                                  &                                                                          & ✓                                                                                      & ✓                                                                                                                                      \\ \hline
\end{tabular}
\end{table*}



\begin{comment}
\begin{table*}[]
\tiny
\centering
\label{tab:relatedworks}
\caption{Related work on the existing research on TD prediction}
\begin{tabular}{l|l|l|l|l|l|l|l}
\hline
                                                                          & \textbf{Tsoukalas et al. {[}10{]}}                                                         & \textbf{Tsoukalas et al. {[}9{]}}                                                              & \textbf{Mathioudaki et al. {[}44{]}}                                  & \textbf{Aversano et al. {[}45{]}}                                  & \textbf{Mathioudaki et al. {[}11{]}}                                  & \textbf{Zozas et al. {[}12{]}}                                                      & \textbf{Our work}                                                                                                                \\ \hline
\textbf{\begin{tabular}[l]{@{}l@{}}Considers \\ seasonality\end{tabular}} &                                                                                            &                                                                                                &                                                                       &                                                                    &                                                                       &                                                                                     & ✓                                                                                                                                \\
\textbf{Feature selection}                                                & \begin{tabular}[l]{@{}c@{}}✓\\ (Correlation analysis,\\ backward elimination)\end{tabular} & \begin{tabular}[l]{@{}c@{}}✓\\ (Hypothesis testing)\end{tabular}                               &                                                                       & \begin{tabular}[l]{@{}c@{}}✓\\ (Correlation analysis)\end{tabular} &                                                                       &                                                                                     & \begin{tabular}[l]{@{}c@{}}✓\\ (Correlation analysis, \\ feature importance, \\ variance thresolding, \\ zero percentage)\end{tabular} \\
\textbf{\begin{tabular}[l]{@{}l@{}}Hyperparameter \\ tuning\end{tabular}} & \begin{tabular}[l]{@{}c@{}}✓\\ (GridSearchCV)\end{tabular}                                 & \begin{tabular}[l]{@{}c@{}}✓\\ (Grid-search method)\end{tabular}                               & \begin{tabular}[l]{@{}c@{}}✓\\ (Grid-search method)\end{tabular}      &                                                                    & \begin{tabular}[l]{@{}c@{}}✓\\ (ACF, PACF)\end{tabular}               & \begin{tabular}[l]{@{}c@{}}✓\\ (Backward Stepwise Regression \\ (BSR))\end{tabular} & \begin{tabular}[l]{@{}c@{}}✓\\ (Auto-ARIMA)\end{tabular}                                                                         \\
\textbf{\begin{tabular}[l]{@{}l@{}}Univariate \\ models\end{tabular}}     &                                                                                            & \begin{tabular}[l]{@{}c@{}}✓\\ (Univariate logistic regression)\end{tabular}                   & \begin{tabular}[l]{@{}c@{}}✓\\ (Multi-layer perceptron)\end{tabular}  &                                                                    & \begin{tabular}[l]{@{}c@{}}✓\\ (ARIMA)\end{tabular}                   & \begin{tabular}[l]{@{}c@{}}✓\\ (ARIMA)\end{tabular}                                 & \begin{tabular}[l]{@{}c@{}}✓\\ (ARIMA, SARIMA)\end{tabular}                                                                      \\
\textbf{\begin{tabular}[l]{@{}l@{}}Multivariate \\ models\end{tabular}}   & \begin{tabular}[l]{@{}c@{}}✓\\ (MLR, SGD, SVR...)\end{tabular}                             & \begin{tabular}[l]{@{}c@{}}✓\\ (LR, NB, DT, KNN, \\ SVM, RF, XGB)\end{tabular}                 &                                                                       & \begin{tabular}[l]{@{}c@{}}✓\\ (MLR, BDT, RF)\end{tabular}         & \begin{tabular}[l]{@{}c@{}}✓\\ (ARIMAX)\end{tabular}                  &                                                                                     & \begin{tabular}[l]{@{}c@{}}✓\\ (ARIMAX, SARIMAX, MLR, \\ SGD, SVR, RF, XGB, ...)\end{tabular}                                    \\
\textbf{Industrial survey}                                                & ✓                                                                                          &                                                                                                &                                                                       &                                                                    &                                                                       & ✓                                                                                   & ✓                                                                                                                                \\
\textbf{\begin{tabular}[l]{@{}l@{}}Long-term \\ forecasting\end{tabular}} & \begin{tabular}[l]{@{}c@{}}✓\\ (1 to 40 weeks ahead)\end{tabular}                          &                                                                                                & \begin{tabular}[l]{@{}c@{}}✓\\ (5 to 150 commits ahead)\end{tabular}  &                                                                    & \begin{tabular}[l]{@{}c@{}}✓\\ (4, 8, 12 steps ahead)\end{tabular}    & \begin{tabular}[l]{@{}c@{}}✓\\ (12 iterations ahead)\end{tabular}                   & \begin{tabular}[l]{@{}c@{}}✓\\ (1 to 36 months ahead)\end{tabular}                                                               \\
\textbf{\begin{tabular}[l]{@{}l@{}}Time Series  \\ models\end{tabular}}   &                                                                                            &                                                                                                & \begin{tabular}[l]{@{}c@{}}✓\\ (ARIMA)\end{tabular}                   &                                                                    & \begin{tabular}[l]{@{}c@{}}✓\\ (ARIMA, ARIMAX)\end{tabular}           & \begin{tabular}[l]{@{}c@{}}✓\\ (ARIMA)\end{tabular}                                 & \begin{tabular}[l]{@{}c@{}}✓\\ (ARIMAX, ARIMA+LM, \\ SARIMAX, SARIMA+LM)\end{tabular}                                            \\
\textbf{ML models}                                                        & \begin{tabular}[l]{@{}c@{}}✓\\ (MLR, SGD, SVR...)\end{tabular}                             & \begin{tabular}[l]{@{}c@{}}✓\\ (LR, NB, DT, KNN,\\  SVM, RF, XGB)\end{tabular}                 & \begin{tabular}[l]{@{}c@{}}✓\\ (RF)\end{tabular}                      & \begin{tabular}[l]{@{}c@{}}✓\\ (MLR, BDT, RF)\end{tabular}         &                                                                       &                                                                                     & \begin{tabular}[l]{@{}c@{}}✓\\ (MLR, SGD, SVR, RF, XGB, ...)\end{tabular}                                                        \\
\textbf{DL models}                                                        &                                                                                            &                                                                                                & \begin{tabular}[l]{@{}c@{}}✓\\ (Multi-layer perceptron)\end{tabular}  &                                                                    &                                                                       &                                                                                     &                                                                                                                                  \\
\textbf{Cross-validation}                                                 & \begin{tabular}[l]{@{}c@{}}✓\\ (Walk-Forward Train-Test)\end{tabular}                      & \begin{tabular}[l]{@{}c@{}}✓\\ (Repeated stratified CV)\end{tabular}                           & \begin{tabular}[l]{@{}c@{}}✓\\ (Walk-Forward Train-Test)\end{tabular} & \begin{tabular}[l]{@{}c@{}}✓\\ (Repeated  CV)\end{tabular}         & \begin{tabular}[l]{@{}c@{}}✓\\ (Walk-Forward Train-Test)\end{tabular} & \begin{tabular}[l]{@{}c@{}}✓\\ (Walk-Forward Train-Test)\end{tabular}               & \begin{tabular}[l]{@{}c@{}}✓\\ (Walk-Forward Train-Test)\end{tabular}                                                            \\
\textbf{\begin{tabular}[l]{@{}l@{}}Performance \\ metrics\end{tabular}}   & \begin{tabular}[l]{@{}c@{}}✓\\ (MAPE)\end{tabular}                                         & \begin{tabular}[l]{@{}c@{}}✓\\ (Precision, Recall, F2, \\ AUC, Module inspection)\end{tabular} & \begin{tabular}[l]{@{}c@{}}✓\\ (MAPE, MAE, RMSE)\end{tabular}         & \begin{tabular}[l]{@{}c@{}}✓\\ (RMSE)\end{tabular}                 & \begin{tabular}[l]{@{}c@{}}✓\\ (MAPE, MAE, RMSE)\end{tabular}         & \begin{tabular}[l]{@{}c@{}}✓\\ (MAPE, MAE, RMSE)\end{tabular}                       & \begin{tabular}[l]{@{}c@{}}✓\\ (MAPE, MAE, RMSE)\end{tabular}                                                                    \\
\textbf{Sample size}                                                      & 15 projects                                                                                & 25 projects                                                                                    & 5 projects                                                            & 8 projects                                                         & 5 projects                                                            & 105 projects                                                                        & 14 projects                                                                                                                      \\
\textbf{Results}                                                          & ✓                                                                                          & ✓                                                                                              & ✓                                                                     & ✓                                                                  & ✓                                                                     & ✓                                                                                   & ✓                                                                                                                                \\
\textbf{Scripts}                                                          & ✓                                                                                          & ✓                                                                                              &                                                                       &                                                                    &                                                                       &                                                                                     & ✓                                                                                                                                \\
\textbf{Datasets}                                                         & ✓                                                                                          & ✓                                                                                              &                                                                       & ✓                                                                  &                                                                       & ✓                                                                                   & ✓                                                                                                                                \\ \hline
\end{tabular}
\end{table*}
\end{comment}

% \todo[inline]{vale 4/10 @mikel: please check if I reported right the comparison with \cite{Zozas2023}, thanks}
% \todo[inline, color=green]{Mikel 05/10 @vale Let me know how it looks now.}

% \todo[inline]{vale 3/11 @Mikel: what means TSA?}


%
% \todo[inline]{vale 3/11: we need to carefully and precisely describe the differences between ~\cite{Mathioudaki2022} in terms of model setup.}
% \todo[inline, color=green]{Mikel 05/10 @vale Please check the structure and logic of my changes in the following paragraph + modification of RQ1}
%
% \todo[inline]{@Vale@Davide: Need updated related work given the combined results.}

% \subsection{Empirical Study on SonarQube}
% \label{sec:ESSOnarQube}
% Static Analysis Tools (SATs) examine the code syntax, structure, and data flow to identify issues. They comprehensively analyze the codebase, searching for problematic patterns, coding errors, and potential performance bottlenecks. By detecting these issues early in the development process, static analysis tools help developers catch bugs before they manifest as runtime errors or security vulnerabilities.

% One of the primary benefits of SATs is their ability to identify common coding mistakes and bad programming practices. They can flag issues such as null pointer dereferences, buffer overflows, memory leaks, and race conditions. Developers can address them promptly, resulting in more reliable and secure software.

% Over the years, the use of SATs has become increasingly popular, leading to a growing body of research. This section discusses previous work on SATs, focusing on their usage, rules, and detected problems~\cite{SaarimakiTechDebt2019, LenarduzziMALTESQUE2019, LenarduzziJSS2019, PecorelliEMSE2022,Beller2016}.

% Most studies have examined the detection capabilities of available SATs~\cite{Lenarduzzi2022}, as well as their solving times in different contexts~\cite{Marcilio2019,Lu2018}. A recent study compared the features and popularity of nine tools, providing empirical evidence of their validity to help practitioners and developers choose the most suitable tool based on their needs. However, this study did not evaluate the agreement and precision of the detection.
% Some studies have concentrated on the accuracy of SATs in identifying issues and their effectiveness, as well as their ability to detect problems related to quality attributes like class fault- or change-proneness. An example of such research includes the work of Pecorelli et al.~\cite{PecorelliEMSE2022} and Lenarduzzi et al.~\cite{LenarduzziMALTESQUE2019, LenarduzziJSS2019, Lenarduzzi2022, LenarduzziSANER2019}. An emerging usage of SATs is in detecting anomalies at various levels of code, which has been explored in a study by Tomas et al.~\cite{Tomas2013}.

% There is still a lot of variability in the performance of SATs and their effectiveness in detecting issues in the code~\cite{LenarduzziSANER2019, LenarduzziJSS2019}. While some studies have demonstrated their usefulness, others have highlighted critical issues such as rule classification, severity assignment, and detection accuracy~\cite{Baldassarre2020, LenarduzziESEM, Lenarduzzi2022}. Additionally, evaluating the performance results can be difficult since different tools have different trade-offs in generating false positives and false negatives~\cite{Rutar2004, Lenarduzzi2022}. The issue of precision has also been raised, indicating the need for better clarification in this area. Overall, it seems that more research is needed to better understand the strengths and weaknesses of different SATs and to develop more reliable and effective methods for detecting issues in the code~\cite{liang2010automatic, Lenarduzzi2022}.


